StoryTTS: A Highly Expressive Text-to-Speech Dataset with Rich Textual Expressiveness Annotations

While acoustic expressiveness has long been studied in expressive text-to-speech (ETTS), the inherent expressiveness in text lacks sufficient attention, especially for ETTS of artistic works. In this paper, we introduce StoryTTS, a highly ETTS dataset that contains rich expressiveness both in acoustic and textual perspective, from the recording of a Mandarin storytelling show. A systematic and comprehensive labeling framework is proposed for textual expressiveness. We analyze and define speech-related textual expressiveness in StoryTTS to include five distinct dimensions through linguistics, rhetoric, etc. Then we employ large language models and prompt them with a few manual annotation examples for batch annotation. The resulting corpus contains 61 hours of consecutive and highly prosodic speech equipped with accurate text transcriptions and rich textual expressiveness annotations. Therefore, StoryTTS can aid future ETTS research to fully mine the abundant intrinsic textual and acoustic features. Experiments are conducted to validate that TTS models can generate speech with improved expressiveness when integrating with the annotated textual labels in StoryTTS.

==> content/backup.tex <==
% intro
% which refers to a form of written language that can bring to life the meaning and feeling of the subject matter to be conveyed. This form of text also influences the cadence and rhythm of the speaker's delivery.
% Among these features, semantic ones are the most commonly utilized. 
% Typically, pre-trained language models (PLMs) are employed to extract semantic features from text, which are then integrated into TTS models. 
% Syntactic features, on the other hand, are employed to indicate lexical properties and interrelationships among words in a sentence, including aspects like part-of-speech (POS) and dependency parsing (DP). 
% \cite{paper3} proposed a graph structure to model both semantic and syntactic features. This approach utilized word embeddings extracted from BERT as vertices of the graph and dependencies as edges. The graph was then represented using a Graph Neural Network to capture the semantic information of the text.
% To achieve natural and expressive TTS synthesis, it's essential to convey the expressive stance of the text, which requires identifying the appropriate expressive meaning within it.
% The methods mentioned above often rely on the semantic representations of PLMs or basic syntactic structures, which may not be sufficient to convey expressive information in the text. 
% In \cite{emotion}, significant results were achieved in a text-based emotion prediction task through emotion annotation and feature extraction from children's fairy tale text. This task is recognized as the primary challenge in addressing emotional TTS. 

% LLM
% \begin{table}[h]
% \centering
%   \caption{Specific categories of Sentence Pattern, Scene, and Rhetoric Device in StoryTTS.}
%   \vspace{3pt}
%  \begin{resizebox}{0.9\columnwidth}{!}
%   {
% \begin{tabular}{cl}
% \toprule
% \textbf{Dimension}                                 & \multicolumn{1}{c}{\textbf{Category}}                      \\ \hline
% \multirow{2}{*}{Sentence Pattern}  & Declarative,\ Interrogative              \\
%                                        & Imperative,\ Exclamatory                \\\midrule
% \multirow{2}{*}{Scene}             & Role-playing,\ Aside                     \\
%                                        & Inner monologue                        \\\midrule
% \multirow{4}{*}{Rhetoric Device} & Hyperbole,\ Antithesis,\ Onomatopoeia  \\
%                                        & Simile,\ Personification,\ Quotation    \\
%                                        & Irony,\ Rhetorical question,\ Hypophora \\
%                                        & Rhetorical repetition,\ Transition         \\ \bottomrule
% \end{tabular}
% }
% \end{resizebox}
%   \label{table:label_cate}
% \end{table}

% exp
% the fusion of all expressive labels brings the biggest boost. They are significantly ahead of baseline in both objective and subjective metrics, and their fusion provides the model with more and more accurate information about the imitated characters and scenes, while syntax, rhetorical devices, and emotional coloring complement each other.
% which may be due to the fact that the majority of the sentences in the data are declarative, resulting in limited information learned by the model, and although the scene types are relatively evenly distributed, they are not sufficient to provide the model with enough information due to the large number of different character imitations in the role-playing and inner monologue scenes. 

% conclusion
% We further introduced a labeling framework for textual expressiveness, which can be divided into two steps. First, we analyzed and defined textual expressiveness in StoryTTS, encompassing five distinct dimensions through the fields of linguistics, rhetoric, and literary studies. Following this, we employed large language models and provided them with a few manual annotation examples for batch annotation.
% The resulting corpus comprises 61 hours of consecutive and highly prosodic speech, accompanied by accurate text transcriptions and rich textual expressiveness annotations.
% Our experiments demonstrated that TTS models can produce speech with enhanced expressiveness when integrating the annotated textual expressiveness labels from StoryTTS. 
% In the future, we will focus on how to combine these expressiveness annotations with acoustic expressiveness to further improve expressive speech synthesis.
